Naive Exploration is Optimal for Online LQR

We consider the problem of online adaptive control of the linear quadratic regulator, where the true system parameters are unknown. We prove new upper and lower bounds demonstrating that the optimal regret scales as $\widetilde{\Theta}({\sqrt{d_{\mathbf{u}}^2 d_{\mathbf{x}} T}})$, where $T$ is the number of time steps, $d_{\mathbf{u}}$ is the dimension of the input space, and $d_{\mathbf{x}}$ is the dimension of the system state. Notably, our lower bounds rule out the possibility of a $\mathrm{poly}(\log{}T)$-regret algorithm, which had been conjectured due to the apparent strong convexity of the problem. Our upper bound is attained by a simple variant of $\textit{{certainty equivalent control}}$, where the learner selects control inputs according to the optimal controller for their estimate of the system while injecting exploratory random noise. While this approach was shown to achieve $\sqrt{T}$-regret by (Mania et al. 2019), we show that if the learner continually refines their estimates of the system matrices, the method attains optimal dimension dependence as well. Central to our upper and lower bounds is a new approach for controlling perturbations of Riccati equations called the $\textit{self-bounding ODE method}$, which we use to derive suboptimality bounds for the certainty equivalent controller synthesized from estimated system dynamics. This in turn enables regret upper bounds which hold for $\textit{any stabilizable instance}$ and scale with natural control-theoretic quantities.

==> body/refined_matrix_bounds.tex <==
%!TEX root = ../max_local.tex
\section{Refined Matrix Bounds}

\begin{comment}

\begin{lem}[Two-Scale OLS Estimate]\label{lem:two_scale_self_normalized_bound} Let $\ProjMat \in \R^{d\times d}$ denote a projection matrix onto a subspace of dimension $p$, and fix an orthonormal basis of $\R^d$, $v_{1},\dots,v_d$, such that $v_{1},\dots,v_p$ form an orthonormal basis for the range of $\ProjMat$. Further, fix positive constants $0 < \lambda_1 \le \nu \le \lambda_2$ such that $\nu_1 \le \sqrt{\lambda_1 \lambda_2/2}$, and define the event 
\begin{align*}
\calE := \left\{\matLam_T \succeq  \lambda_1 \ProjMat +  \lambda_2 (I-\ProjMat) \right\} \cap \left\{\|\ProjMat \matLam_T (1-\ProjMat)\|_{\op} \le \nu\right\}
\end{align*} 
Then, with probability $1 - \delta$, if $\calE$ holds, 
\begin{align*}
\|\Thetahat_T - \Thetast \|_\fro^2 \le  \frac{12 mp \matkappa_1 }{\lambda_1}  \log \frac{3 md \matkappa_1}{ \delta} + \left(\frac{\nu}{\lambda_1}\right)^2 \cdot \frac{48m(p-d)\matkappa_2 }{\lambda_2}\log \frac{3 md\matkappa_2}{ \delta}. 
\end{align*}
where $\matkappa_1:= \max_{1 \le j \le p} v_j^\top \matLam_T v_j / \lambda_2$ and $\matkappa_2 := \max_{p+1 \le j \le d} v_j^\top \matLam_T v_j / \lambda_1$. 
\end{lem}
\end{comment}

\subsection{Bounding the Cross Term}

\begin{proof}
\newcommand{\matxring}{\mathring{\matx}}
\newcommand{\matxch}{\check{\matx}}
Consider a fixed epoch $k$, and for $t\in \{\tau_{k},\tau_{k} + 1, \dots,\tau_{k+1}-1\}$, introduce the contribution from all previous steps:
\begin{align*}
\matxring_t := \Exp[\matx_t \mid \calF_{\tau_{k}}] = \Aclk^{t-\tau_{k}}\matx_{\tau_{k}}l
\end{align*} 
 where $(\calF_{t})$ is the filtration generated by $\matx_{1:t-1},\matw_{1:t-1},\matu_{1:t-1}$, and where the equality follows from direct computation. Further, introduce the difference  
 \begin{align}
 \matxch_t := \matx_t - \matxring_t, \label{eq:matxch}
 \end{align} 
 The important observation here is
 \begin{obs}\label{obs:matxch_linear} $\matxch_t$ is a linear form in the jointly standard-normal Gaussian vector $\matgbar := (\matw_t,\matg_t : \tau_k \le t \le \tau_{k+1}-1)$. 
 \end{obs} We then have 
\begin{align*}
\ProjMat_k \matLam_k (I - \ProjMat_k) &= \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix}\matx_t  \\\matu_t
\end{bmatrix} \begin{bmatrix}\matx_t  \\\matu_t
\end{bmatrix}^\top (I - \ProjMat_k)\\
%
&= \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix}\matx_t \\\Khat_k \matx_t + \sigma_k \matg_t
\end{bmatrix} \begin{bmatrix}\matx_t \\\Khat_k \matx_t + \sigma_k \matg_t
\end{bmatrix}^\top  (I - \ProjMat_k)\\
%
&\overset{(i)}{=} \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix} 0 \\  \sigma_k \matg_t
\end{bmatrix} \begin{bmatrix}\matx_t \\\Khat_k \matx_t + \sigma_k \matg_t
\end{bmatrix}^\top  (I - \ProjMat_k)\\
%
&\overset{(ii)}{=}  \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix} 0 \\  \sigma_k \matg_t
\end{bmatrix} \begin{bmatrix} \matxch_t \\  \Khat_k \matxch_t \end{bmatrix}^\top  (I - \ProjMat_k) + 
%
\sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix} 0 \\  \sigma_k \matg_t
\end{bmatrix} \begin{bmatrix} \matxring_t \\  \Khat_k \matxring_t \end{bmatrix}^\top  (I - \ProjMat_k)
\\\
&\quad+ \sigma_k^2\sum_{t = \tau_{k}}^{\tau_{k+1}-1} \ProjMat_k \begin{bmatrix} 0 & 0 \\
 0 & \matg_t \matg_t^\top \end{bmatrix} (I - \ProjMat_k),
\end{align*}
where here $(i)$ follows since $\ProjMat_k$ annihilates the subspace $(x,u) : u = Kx$, and where $(ii)$ decomposes using linearity. Since $\|\ProjMat_k\|_{\op} \vee \|I - \ProjMat_k\|_{\op} \le 1$, we can upper bound, we bound the operator norm of $\nrm*{\ProjMat_k \matLam_k (I - \ProjMat_k)}_{\op}$ by three terms:
\newcommand{\term}{\mathsf{term}}

\begin{multline*}
\nrm*{\ProjMat_k \matLam_k (I - \ProjMat_k)}_{\op} \le  \\
 \sigma_k \underbrace{\nrm*{\sum_{t = \tau_{k}}^{\tau_{k+1}-1} \matg_t
 \begin{bmatrix} \matxch_t\mid  \Khat_k \matxch_t \end{bmatrix} }_{\op}}_{\term_1} + \sigma_k  \underbrace{ \nrm*{\sum_{t = \tau_{k}}^{\tau_{k+1}-1}  \matg_t \begin{bmatrix} \matxring_t\mid  \Khat_k \matxring_t \end{bmatrix} }_{\op}}_{\term_2} + \sigma_k^2  \underbrace{ \nrm*{\sum_{t = \tau_{k}}^{\tau_{k+1}-1} \matg_t \matg_t^\top }_{\op}}_{\term_3}.
\end{multline*}
Let us bound each term in order;

\paragraph{Bounding $\term_1$}
\newcommand{\Tleft}{\mathcal{T}_{\mathrm{left}}}
\newcommand{\Tright}{\mathcal{T}_{\mathrm{right}}}
\begin{defn}[Relevant $\epsilon$-nets]\label{defn:relevant_epsilon_nets}
Let $\Tleft$ be an $1/4$-net of the unit ball in $\R^\dimu$, and let $\Tright$ be a $1/4$-net of the unit ball in the subsapce $\R^{\dimx + \dimu}$ spanned by $(I - \ProjMat_k)$, that is, spanned by vectors of the form $(x,\Khat_k x)$. We use $w$ to denote elements of $\Tleft$, and $v = (v_1,v_2)$ to denote elements of this net $\Tright$, partitioned into the $\R^{\dimx}$ and $\R^{\dimu}$ components.
\end{defn}

A standard covering argument entails that 
\begin{align*}
\term_1 \lesssim \max_{w \in \Tleft, v = (v_1,v_2) \in \Tright} \term_1(w,v)\quad \text{where }  \term_1(w,v) := \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \langle w, \matg_t\rangle
\langle (\matxch_t,\Khat_k \matxch_t), v \rangle.
\end{align*}
From \Cref{obs:matxch_linear}, $\term_1(w,v)$ is a quadratic form in a Gaussian vector $\matgbar = ((\matw_t,\matg_t) : \tau_{k} \le t \le \tau_{k+1} - 1)$ encoding both input noise $\matg_t$ and process noise $\matw_t$, and thus may express that for some matrix $Q(w,v)$, which without loss of generality we can choose to be symmetric, for which 
\begin{align*}
  \term_1(w,v) = \matgbar^\top Q(w,v)\matgbar
\end{align*}
When clear from context, we abridge $Q = Q(w,v)$. 

We shall apply the Hanson Wright inequality, which requires bounding $\tr(Q)$, $\|Q\|_{\fro}$, and $\|Q\|_{\op}$. We first see that $\tr(Q) = 0$, since $\Exp[\term_1(w,v)] = 0$, as the noise $\matg_t$ is independent of $\matxch_t$. Moreover, we can bound $\|Q\|_{\fro} \le \sqrt{\rank(Q)}\|Q\|_{\op}$. To bound $\rank(Q)$:
\begin{claim}\label{claim:Q_rank} $\rank(Q) \le \tau_{k}$, and thus $\|Q\|_{\fro} \le \sqrt{\tau_{k}}\|Q\|_{\op}$
\end{claim}
\begin{proof}[Proof of \Cref{claim:Q_rank}] Let $X_{t} : \R^{\dim(\matgbar)} \to  \R^{\dimu}$ denote the projection matrix yielding $X_t \matgbar = \matg_t$, and let  $Y_t := \R^{\dim(\matgbar)} \to \R^{\dimx + \dimu}$ denote the linear operator $Y_t \matgbar = (\matxch_t,\Khat_k \matxch_t)$; these are indeed linear by \Cref{obs:matxch_linear}, namely that $\matxch_t = \matx_t - \matxring_t$ is linear in the noise vector $\matgbar$.

Let $\bar{X} := X_t$ denote the matrix whose rows are $X_{\tau_{k}},\dots, X_{\tau_{k+1} - 1}$, and let $\bar{Y}$ be analogous. Then, 
\begin{align*}
\matgbar^\top Q(w,v)\matgbar &= \term_1(w,v) \\
&= \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \matg_t^\top w v^\top
 (\matxch_t,\Khat_k \matxch_t), v  = \sum_{t=\tau_{k}}^{\tau_{k+1}} \matgbar^\top X_t^\top wv^\top Y_t \matgbar \\
 &= \matgbar\bar{X}\Diag_{\tau_{k}(wv^\top)}\bar{Y}\matgbar,
\end{align*}
where $\Diag_{\tau_{k}(wv^\top)}$ denotes the block-diagonal matrix consisting of $\tau_k$ blocks of the rank-one terms $wv^\top$. Hence, the quadratic form $Q$ can be rendered explicitly as $Q = \bar{X}\Diag_{\tau_{k}}(wv^\top)\bar{Y}$, which has rank at most $\rank(\Diag_{\tau_{k}}(wv^\top)) = \tau_{k} \cdot \rank(wv^\top) = \tau_{k}$. 
\end{proof}
\newcommand{\Qbar}{\bar{Q}}
Next, we bound  $\|Q\|_{\op}$. 
\begin{claim} $\opnorm{Q} \lesssim \opnorm{\Pst}^{5/4}$
\end{claim}
\begin{proof} We construct a matrix $\Qbar \succeq 0$ such that $-\Qbar \preceq Q \preceq \Qbar$. It follows that $\|Q\|_{\op} \le \Qbar$
Let us contrinue by constructing $\Qbar$. For any parameter $\alpha > 0$, 
\begin{align*}
\term_1(w,v) := \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \langle w, \matg_t\rangle
\langle (\matxch_t,\Khat_k \matxch_t), v \rangle &\le \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \frac{\alpha}{2} \matg_t^\top ww^\top \matg_t + \frac{1}{2\alpha}(\matxch_t,\Khat_k \matxch_t)^\top vv^\top(\matxch_t,\Khat_k \matxch_t)^\top \\
&\overset{(i)}{\le} \frac{\alpha}{2}\underbrace{\sum_{t = \tau_{k}}^{\tau_{k+1}-1} \matg_t^\top ww^\top \matg_t}_{:= \matgbar^\top \Qbar_1(w,v) \matgbar} + \frac{1}{\alpha} \underbrace{\sum_{t = \tau_{k}}^{\tau_{k+1}-1}  \matxch_t^\top (v_1 v_1^\top + \Khat_k v_2 v_2 \Khat_k^\top)\matxch_t}_{:= \matgbar^\top \Qbar_2(w,v) \matgbar} \\
&\overset{(ii)}{:=} \matgbar^\top \Qbar(w,v) \matgbar
\end{align*}
where in $(i)$, we use the decompose $v = (v_1,v_2)$ as in \Cref{defn:relevant_epsilon_nets}, and use the elementary inequality $vv^\top \preceq \begin{bmatrix} v_1 v_1^\top & 0 \\ 0 & v_2 v_2^\top \end{bmatrix}$. In $(ii)$, we again invoke that $\matxch_t$ is linear in $\matgbar$ (\Cref{obs:matxch_linear}).

Since the above inequality holds for any realization of the noise,  we find that $Q(w,v) \preceq   \Qbar(w,v)$, and a similar manipulation shows that $Q(w,v) \succeq - \Qbar(w,v)$. Noting that $\|Q(w,v)\|_{\op} \le \|\Qbar(w,v)\|_{\op} = \| \frac{\alpha}{2}\Qbar_1(w,v) + \frac{1}{\alpha}\Qbar_2(w,v)\|_{\op} \le \frac{\alpha}{2}\|\Qbar_{1}(w,v)\|_{\op} +\frac{1}{\alpha}  \|\Qbar_2(w,v)\|_{\op}$, we bound $\|\Qbar_{1}(w,v)\|_{\op}$ and $\|\Qbar_2(w,v)\|_{\op}$. We have first that, deterministically,
\begin{align*}
\matgbar^\top \Qbar_1(w,v) \matgbar = \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \matg_t^\top ww^\top \matg_t \le \sum_{t = \tau_{k}}^{\tau_{k+1}-1}\|\matg_t\|^2 \le \sum_{t = \tau_{k}}^{\tau_{k+1}-1}\|\matg_t\|^2 + \|\matw_t\|^2 = \|\matgbar\|^2,
\end{align*}
so that $\|\Qbar_1(w,v)\|_{\op} \le 1$. Moreover, by applying \Cref{lem:quadratic_forms_cost} with $x_1 = 0$, $R_2 = 0$, $\sigma_u = \sigma_k$,  $R_1 = v_1 v_1^\top + \Khat_k v_2 v_2 \Khat_k^\top$, we can bound 
\begin{align*}
 \|\Qbar_2(w,v)\|_{\op} &\lesssim (1 + \sigma_k^2 \|\Bst\|_{\op}^2)\|\Ast + \Bst \Khat_k\|_{\Hinfty}\|R_1\|_{\op}\\
 &\lesssim (1 + \sigma_k^2 \|\Bst\|_{\op}^2)\|\Ast + \Bst \Khat_k\|_{\Hinfty}(1 + \|\Khat_k\|_{\op}^2).
\end{align*}
In particular, for $\sigma_k \le 1/\Psibst^2$, we have $(1 + \sigma_k^2 \|\Bst\|_{\op}^2) \lesssim 1$, and and nder the safe event $\Esafe$, we have $\|\Khat_k\|^2_{\op} \le \frac{21}{20}\opnorm{\Pst}$  and $\|\Ast + \Bst \Khat_k\|_{\Hinfty} := \|\Aclk\|_{\Hinfty} \le \opnorm{\Pst}^{3/2}$. Since $\opnorm{\Pst} \ge 1$, this allows us to bound 
\begin{align*}
 \|\Qbar_2(w,v)\|_{\op} \lesssim \opnorm{\Pst}^{5/2},
\end{align*}
provided again that $\sigma_k \le \Psibst$. Hence, setting $\alpha = \opnorm{\Pst}^{5/4}$, 
\begin{align*}
\|Q(w,v)\|_{\op} \le \frac{\alpha}{2} \|\Qbar_1(w,v)\|_{\op} + \frac{1}{\alpha} \|\Qbar_2(w,v)\|_{\op} \lesssim \frac{\alpha}{2} + \frac{1}{\alpha}\opnorm{\Pst^{5/2}} \lesssim \opnorm{\Pst}^{5/4}. 
\end{align*}
\end{proof}
Gathering the past two claims, we have $\|Q\|_{\op} \lesssim \opnorm{\Pst}^{5/4}$ and $\|Q\|_{\fro} \lesssim \sqrt{\tau_{k+1}}\opnorm{\Pst}^{5/4}$. Hence, the Hanson-Wright Inequality implies that, for some universal constant $c>0$,
\begin{align*}
\Pr\left[ \term_1(w,v) \ge c\opnorm{\Pst}^{5/4}\left(\sqrt{\tau_{k+1}} \log(1/\delta) + \log(1/\delta) \right) \right] \le \delta.
\end{align*}
Finally, taking a union bound over $w \in \Tleft$ and $v \in \Tright$, and noting that we may choose $\log |\Tleft||\Tright| \lesssim \dimx + \dimu$, we have for $\tau_{k+1} \ge \dimx + \dimu + \log(1/\delta)$ and another universal constant $c$ that
\begin{align*}
\Pr\left[ \sup_{v \in \Tleft,w \in \Tright} \term_1(w,v) \ge c\opnorm{\Pst}^{5/4}\sqrt{\tau_{k+1} (\dimx + \dimu + \log(1/\delta)} \right] \le \delta.
\end{align*}
Finally, by a standard covering argument (\mscomment{cite}), this implies that for another constant $c$,
\begin{align*}
\Pr\left[ \term_1 \ge c\opnorm{\Pst}^{5/4}\sqrt{\tau_{k+1} (\dimx + \dimu + \log(1/\delta)} \right] \le \delta.
\end{align*}

\paragraph{Bounding $\term_2$}
Again, we use a covering argument. with $\Tleft$ be an $1/4$-net of the unit ball in $\R^\dimu$, and let $\Tright$ be a $1/4$-net of the unit ball in the subspace $\R^{\dimx + \dimu}$ spanned by $(I - \ProjMat_k)$. Similarly, use 
\begin{align*}
\term_2 \lesssim \max_{w \in \Tleft, v = (v_1,v_2) \in \Tright} \term_2(w,v)\quad \text{where }  \term_2(w,v) := \sum_{t = \tau_{k}}^{\tau_{k+1}-1} \langle w, \matg_t\rangle
\langle (\matxring_t,\Khat_k \matxring_t), v \rangle.
\end{align*}
Since $\matxring_t =  \Aclk^{t-\tau_{k}}\matx_{\tau_{k}}$, we see that $(\matg_t : t \ge \tau_{k})$ are independent of the terms $\langle (\matxring_t,\Khat_k \matxring_t), v \rangle$. Since $\|v\| = 1$,  $\langle w, \matg_t \rangle$ are then independent standard Gaussian random vectors. Hence, by standard Gaussian tail bound, 
\begin{align*}
\term_2(w,v)  \le \sqrt{2 \sum_{t=\tau_{k}}^t 
\langle (\matxring_t,\Khat_k \matxring_t), v \rangle^2 \log(1/\delta)}, \text{ w.p. } 1 - \delta.
\end{align*}
\begin{claim} $ \sum_{t=\tau_{k}}^t \langle (\matxring_t,\Khat_k \matxring_t), v \rangle^2  \le $
\end{claim}
\begin{proof}
We can bound
\begin{align*}
\sum_{t=\tau_{k}}^t 
\langle (\matxring_t,\Khat_k \matxring_t), v \rangle^2 &= v^\top\begin{bmatrix} I \\ \Khat_k \end{bmatrix}^\top \sum_{t=\tau_{k}}^t \matxring_t \matxring_t^\top \begin{bmatrix} I \\ \Khat_k \end{bmatrix}v \le \nrm*{\sum_{t=\tau_{k}}^t \matxring_t \matxring_t^\top}_{\op} \|v\|^2 \nrm*{\begin{bmatrix} I \\ \Khat_k \end{bmatrix}}^2 \\
&= (1 + \|\Khat_k\|^2) \nrm*{\sum_{t=\tau_{k}}^t \matxring_t \matxring_t^\top}_{\op} \le (1 + \|\Khat_k\|^2)\tr\left(\sum_{t=\tau_{k}}^t \matxring_t \matxring_t^\top\right).
\end{align*}
Furthermore, since $\matxring_t = \Acl^{t-\tau_{k+1}}\matx_{\tau_{k}}$, a standdard computation shows that 
\begin{align*}
\sum_{t=\tau_{k}}^t \matxring_t \matxring_t^\top \le  \matx_{\tau_{k}}^\top \dlyap(\Aclk,I)\matx_{\tau_{k}} \le \matx_{\tau_{k}}^\top P_k\matx_{\tau_{k}}
\end{align*}
\end{proof}

\paragraph{Bounding $\term_3$}
From \mscomment{Vershynin}, we have that if $\tau_{k+1} - \tau_{k} = \tau_{k} \gtrsimst d \log(1/\delta)$ 



\end{proof}

\begin{comment}
\begin{lem}[Matrix Freedman's Inequality,  Theorem 1 in  \citet{tropp2011freedman}] Let $Y_t$ denote a matrix martingale adapted to a filtration $\calF_t$, and let $X_t$ denote the associated martingale increments. Assume that $- R I  \preceq X_t \preceq RI$, define the variance process
\begin{align*}
W_{t,1} := \Exp\left[\sum_{s=1}^t X_sX_s^\top \mid \calF_{s-1}\right], \quad W_{t,2} := \Exp\left[\sum_{s=1}^t X_s^\top X_s \mid \calF_{s-1}\right]
\end{align*}
Then, for an $\sigma^2 > 0$ and $t > 0$, that
\begin{align*}
\Pr[ \exists t: \lambda_{\max}(Y_t) \ge u \text{ and }  W_t \preceq \sigma^2 I] \le d\exp( - \frac{u^2/2}{\sigma^2 + Ru/3}).
\end{align*}
In particular, if $\|W_T\| \preceq \sigma^2 T $ almost surely, then with probability $1 - \delta$,
\begin{align*}
\Pr\left[\frac{1}{T}\|Y_T\|_{\op} \ge  \sqrt{\frac{2\sigma^2 \log (2d/\delta)}{T}} + \frac{2R^2 \log(2d/\delta)}{3T}\right] \le \delta.
\end{align*}
\end{lem} 
\begin{proof} For a given $k$, define the martingale sequence $Y_i := \ProjMat_k \matz_{i+\tau_{k+1}} \matz_{i+\tau_{k+1}} (I - \ProjMat)$. We can develop
\begin{align*}
Y_i &:= \ProjMat_k \matz_{i+\tau_{k+1}} \matz_{i+\tau_{k+1}} (I - \ProjMat) + \\
&:= \ProjMat_k \begin{bmatrix} \matx_{i+\tau_{k+1}}\\
\matu_{i+\tau_{k+1}}\end{bmatrix} \begin{bmatrix} \matx_{i+\tau_{k+1}}\\
\matu_{i+\tau_{k+1}}\end{bmatrix}^\top (I - \ProjMat)
\end{align*}
\end{proof}
\end{comment}



\begin{comment}
\subsection{ Proof of \Cref{lem:two_scale_self_normalized_bound}}
	We begin with a linear algebraic lemma lower bounding the square of a PSD matrix in the Lowner order.

		\begin{lem}\label{lem:matrix_sq_lb}
			Let $X = \begin{bmatrix} X_{11} & X_{12} \\
			X_{12}^\top & X_{22}\end{bmatrix} \succ 0$. Then, 
			\begin{align*}
			X^2  &\succeq \begin{bmatrix} ( 1- \alpha_1) X_{11}^2  + (1 - \alpha_2^{-1}) X_{12}X_{12}^\top & 0\\
			%
			0 & (1 - \alpha_2) X_{22}^2 +(1 - \alpha_1^{-1}) X_{12}^\top X_{12} \end{bmatrix}
			\end{align*}
		\end{lem}
		\begin{proof}[Proof of \Cref{lem:matrix_sq_lb}]
			
			We begin by expanding
			\begin{align*}
			\begin{bmatrix} X_{11} & X_{12} \\
			X_{12}^\top & X_{22}\end{bmatrix}^2 &= \begin{bmatrix} X_{11}^2 + X_{12}X_{12}^\top & X_{11}X_{12} + X_{12}X_{22} \\
			%
			X_{22} X_{12}^\top + X_{12}^\top X_{11}& X_{22}^2 + X_{12}^\top X_{12}\end{bmatrix}\\
			%
			& = \begin{bmatrix} X_{11}^2 + X_{12}X_{12}^\top & 0\\
			%
			0 & X_{22}^2 + X_{12}^\top X_{12}\end{bmatrix} 
			+ \begin{bmatrix} 0 & X_{11} X_{12} \\
			X_{12}^\top X_{11} & 0 
			\end{bmatrix} + \begin{bmatrix} 0 &  X_{12} X_{22} \\
			 X_{22}X_{12}^\top & 0 
			\end{bmatrix} .
			\end{align*}
			Now, for any vector $v = (v_1,v_2)$, and any $\alpha_1 > 0$, we have 
			\begin{align*}
			\left\langle v, \begin{bmatrix} 0 & X_{11} X_{12} \\
			X_{12}^\top X_{11}
			\end{bmatrix} v \right \rangle  &= 2v_1^\top X_{11} X_{12} v_2 \\
			&\ge -  2\|v_1^\top X_{11}\| \|X_{12} v_2\| \\
			&= -  2 \cdot \alpha_1^{1/2}\|v_1^\top X_{11}\| \cdot \alpha_1^{-1/2}\|X_{12} v_2\|\\ 
			&\ge -\alpha_1 \|v_1^\top X_{11}\|^2 - \alpha_1^{-1} \|X_{12} v_2\|^2\\
			&= \left\langle v, \begin{bmatrix} - \alpha_1 X_{11}^2 & 0\\
			0 & - \alpha_1^{-1} X_{12}^\top X_{12}
			\end{bmatrix} v \right\rangle.
			\end{align*}
			Similarly, for any $v$ and $\alpha_2 > 0$, we have
			\begin{align*}
			\left\langle v, \begin{bmatrix} 0 & X_{12} X_{22} \\
			X_{22} X_{12}^\top
			\end{bmatrix} v \right \rangle 
			&\ge \left\langle v, \begin{bmatrix} - \alpha_2^{-1}  X_{12} X_{12}^\top & 0\\
			0 & - \alpha_2 X_{22}^2
			\end{bmatrix} v \right\rangle.
			\end{align*}
			Thus, for any $\alpha_1,\alpha_2 > 0$, 
			\begin{align*}
			X^2  &\succeq \begin{bmatrix} ( 1- \alpha_1) X_{11}^2  + (1 - \alpha_2^{-1}) X_{12}X_{12}^\top & 0\\
			%
			0 & (1 - \alpha_2) X_{22}^2 +(1 - \alpha_1^{-1}) X_{12}^\top X_{12} \end{bmatrix}
			\end{align*}
		\end{proof}

	The important case of \Cref{lem:matrix_sq_lb} is when the matrix $X$ in question can be lower bounded in terms of the weighted sum of two complementary projection matrices.
		\begin{lem}\label{lem:proj_matrix_cond} 
			Let $\ProjMat$ be an orthogonal projection matrix, let $X \succ 0$, and suppose that there exist positive constants $\lambda_1 \le \nu \le \lambda_2$ be such that   $X \succeq \lambda_1 (I-\ProjMat) + \lambda_2 \ProjMat$, and $\|\ProjMat X (1-\ProjMat)\|_{\op} \le \nu$. Then, if $\nu \le \sqrt{\lambda_1 \lambda_2}/2$, 
			\begin{align*}
			X^2 \succeq \frac{1}{4} \lambda_{1}^2 \ProjMat + \frac{\lambda_{1}^2 \lambda_2^2}{16\nu^2}  (I - \ProjMat) 
			\end{align*}
		\end{lem}
		\begin{proof}[Proof of \Cref{lem:proj_matrix_cond}]

			Denote the number of rows/columns of $X$ by $d$. By an orthonormal change of basis, we may assume that $\ProjMat$ is the projection onto the first $k = \dim(\range(\ProjMat))$ cannonical basis vectors. Writing $X$ and $\ProjMat$ in this basis we have
			\begin{align}
			X = \begin{bmatrix} X_{11} & X_{12} \\
			X_{12}^\top & X_{22}\end{bmatrix} \succeq \lambda_1 (I-\ProjMat) + \lambda_2 \ProjMat =  \begin{bmatrix} \lambda_1 I_{d -p} & 0 \\
			0 &  \lambda_2 I_k \end{bmatrix}. \label{eq:X_in_basis}
			\end{align}
			It suffices to show that, in this basis
			\begin{align}
			X^2  &\succeq \begin{bmatrix} \frac{\lambda_1^2}{4} I_p & 0\\
			%
			0 & \frac{\lambda_2^2\lambda_1^2}{16\nu^2}  I_{d-p} \end{bmatrix}. \label{eq:X_Squared_tws}
			\end{align}
			From \Cref{eq:X_in_basis}, $X_{11} \succeq \lambda_1 I_{p} $, $X_{22} \succeq \lambda_2 I_{p-d}$, and $\|X_{12}\|_{\op} = \|\ProjMat X (1-\ProjMat)\|_{\op}$. Hence, hence the parameters $\nu \ge \lambda_1$ in the lemma satisfies $\nu \ge \|X_{12}\|_{\op}$. Thus, 
			\begin{align*}
			X^2  &\succeq \begin{bmatrix} \left\{( 1- \alpha_1)  + (1 - \alpha_2^{-1}) (\nu/\lambda_1)^2 \right\} \cdot \lambda_1^2 I_p & 0\\
			%
			0 & \left\{(1 - \alpha_2)  +(1 - \alpha_1^{-1}) (\nu/\lambda_2)^2\right\} \cdot \lambda_2^2 I_{d-p} \end{bmatrix}.
			\end{align*}
			Set $\alpha_1 = \frac{1}{2}$, and take  $\alpha_2$ to satisfy $(1 - \alpha_2^{-1})(\nu/\lambda_1)^2 = -1/4$. Then, we have the following string of implicitations
			\begin{align*}
			1 - \alpha_2^{-1} &= -\lambda_1^2/4\nu^2 \quad \implies \quad
			\alpha_2^{-1} = \frac{4 \nu^2 + \lambda_1^2}{\nu^2} \quad \implies\\
			\alpha_2 &= \frac{4\nu^2}{4\nu^2 + \lambda_1^2} \quad \implies \quad
			1 - \alpha_2 = \frac{\lambda_1^2}{4 \nu^2 + \lambda_1^2} \ge \frac{\lambda_1^2}{8 \nu^2},
			\end{align*} 
			where in the last line we use $\nu \ge \lambda_1$. For this choice, and using $\nu \le \sqrt{\lambda_1 \lambda_2}/2$,
			\begin{align*}
			X^2  &\succeq \begin{bmatrix} \frac{\lambda_1^2}{4} I_p & 0\\
			%
			0 & \{\frac{\lambda_1^2}{8 \nu^2}  - \frac{\nu^2}{\lambda_2^2}\} \cdot \lambda_2^2 I_{d-p} \end{bmatrix} \succeq \begin{bmatrix} \frac{\lambda_1^2}{4} I_p & 0\\
			%
			0 & \frac{\lambda_2^2\lambda_1^2}{16\nu^2}  I_{d-p} \end{bmatrix}, 
			\end{align*}
			as needed.
		\end{proof}

	We are now in a position to prove our desired lemma.
		\begin{proof}[Concluding the proof of \Cref{lem:two_scale_self_normalized_bound}]
			
			Let's establish the following notation:
			\begin{itemize}
				\item We assume without loss of generality that $\sigma^2 = 1$. 
				\item Let $\mate_t = \maty_t - \Thetast\matz_t$. Let $\matE \in \R^{Td}$ denote the matrix whose rows are $\mate_t$, and $\matE^{(i)} \in \R^T$ denote the vector $(\mate_{1,i},\dots,\mate_{T,i})$, where $\mate_{t,i}$ is the $i$-th coordinate of $\mate_t$.
				\item Recall that $v_{1,\dots,p}$ denote a basis for the range of the projection operator $\ProjMat$, and $v_{p+1,\dots,d}$ complete this basis to form an orthonormal basis for $\R^d$.
			\end{itemize}
			

			 By the assumptions that $\matLam_T \succeq \lambda_1 (I-\ProjMat) + \lambda_2 \ProjMat$, and $\nu \ge \lambda_1 \vee \|\ProjMat \matLam_T (1-\ProjMat)\|$, and $\nu \le \sqrt{\lambda_1 \lambda_2}/2$, \Cref{lem:proj_matrix_cond} implies that 
			\begin{align*}
			\matLam_T^2  \succeq \frac{1}{4} \lambda_{1}^2 \ProjMat + \frac{\lambda_{1}^2 \lambda_2^2}{16\nu^2}  (I - \ProjMat) 
			\end{align*} 
			so after inversion, 
			\begin{align*}
			(\matX_T^\top \matX_T)^{-2} \preceq 4\lambda_{-1}^2 \ProjMat + \frac{16\nu^2}{\lambda_{1}^2 \lambda_2^2}  (I - \ProjMat).
			\end{align*}
			Hence, we can render
			\begin{align*}
			\|\Thetahat_T - \Thetast \|_\fro^2 &= \sum_{i=1}^m \left\|(\matX^\top \matX)^{-1} \matX^\top \matE^{(i)} \right\|_{2}^2 \\
			&= \sum_{i=1}^m \left \langle \matX^\top \matE^{(i)} , (\matX^\top \matX)^{-2} \matX^\top \matE^{(i)} \right \rangle \\
			%
			&\le \sum_{i=1}^m \left \langle \matX^\top \matE^{(i)} , \left(4\lambda_{1}^{-2} \ProjMat + \frac{16\nu^2}{\lambda_{1}^2 \lambda_2^2}  (I - \ProjMat)\right) \matX^\top \matE^{(i)} \right \rangle \\
			%
			&= \sum_{i=1}^m 4\lambda_{1}^{-2}\|\ProjMat \matX^\top \matE^{(i)}\|^2 +  \frac{16\nu^2}{\lambda_{1}^2 \lambda_2^2}  \|(I - \ProjMat) \matX^\top \matE^{(i)}\|^2 \\  
			&= \sum_{i=1}^m  \frac{4}{\lambda_1^2} \left(\sum_{j=1}^p  \left\langle v_j, \matX^\top \matE^{(i)} \right\rangle^2\right) + \frac{16\nu^2}{\lambda_{1}^2 \lambda_2^2} \left(\sum_{j=p+1}^d   \left\langle v_j ,\matX^\top \matE^{(i)}\right\rangle^2\right)  
			\end{align*}
			\newcommand{\symv}{\boldsymbol{v}}
			For an index $j$, let $\lambda[j]$ equal $\lambda_1$ if $j \le p$, and $\lambda_2$ if $ p + 1 \le d \le d $, and define the vector $\matX_j = \matX v_j$. Then, $\left\langle v_j, \matX^\top \matE^{(i)} \right\rangle^2$ can be bounded as  as 
			\begin{align*}
			\left\langle v_j, \matX^\top \matE^{(i)} \right\rangle^2 &= \|\matX_j^\top \matE^{(i)}\|_2^2\\
			&= \|\matX_j\|^{2} \cdot \frac{\left\| \matX_j^\top \matE^{(i)}\right\|_2^2}{\|\matX_j\|_2^{2}}\\
			&\le \|\matX_j\|^{2} \cdot \frac{3}{2} \frac{\left\| \matX_j^\top \matE^{(i)}\right\|_2^2}{\|\matX_j\|_2^2 + \frac{1}{2}\lambda[j]},
			\end{align*}
			where in the last inequality we use that $\|\matX_j\|_2^2 = v_j^\top \matLam_T v_j \ge v_j^\top (\lambda_1 (1-\ProjMat) + \lambda_2 \ProjMat) v_j = \lambda[j]$. 

			By the scalar-valued  self normalized tail inequality~\Cref{lem:self_normalized},  it holds with probability $1-\delta$ that 
			\begin{align*}
			\left\langle v_j, \matX^\top \matE^{(i)} \right\rangle^2 &\le   3\|\matX_j\|_2^2 \log \frac{\frac{1}{2}\lambda[j] + \|\matX_j\|_2^2}{\frac{1}{2}\lambda_j[j]\delta}\\
			&\le   3\lambda[j] \matkappa[j] \log \frac{\frac{1}{2}\lambda[j] + \lambda[j] \matkappa[j]}{\frac{1}{2}\lambda_j[j]\delta}\\
			&\le   3\lambda[j] \matkappa[j] \log \frac{3 \matkappa[j]}{\delta}\\
			&= \begin{cases} 3\lambda_1 \matkappa_1  \log \frac{3 \matkappa_1}{\delta} & j \le d \\
			3\lambda_2 \matkappa_2  \log \frac{3 \matkappa_2}{\delta} & j \ge d \\
			\end{cases}
			\end{align*}
			where we set $\matkappa[j] := \frac{v_j^\top \matLam_Tv_j}{\lambda[j]} \ge 1 $, and note that $\matkappa_1 := \max_{1 \le j \le d} \matkappa[j]$ and $\matkappa_2 := \max_{j > p} \matkappa[j]$. Hence, taking a union bound over all $dm$ coordinates
			\begin{align*}
			& \|\Thetahat_T - \Thetast \|_\fro^2\\
			 &\quad\le \sum_{i=1}^m  \frac{4}{\lambda_1^2} \left(\sum_{j=1}^p 3\lambda_1 \matkappa_1 \log \frac{3 dm\matkappa_1}{ \delta}\right) + \frac{16\nu^2}{\lambda_{1}^2 \lambda_2^2} \left(\sum_{j=p+1}^d   3\lambda_2 \matkappa_2 \log \frac{3 dm\matkappa_2}{ \delta}\right)  \\
			%& \sum_{i=1}^m \frac{8 + 2 \nu_2^2}{\lambda_{1}^2} \left(\sum_{j=p+1}^d  +  \frac{4}{\lambda_2^2} \left(\sum_{j=1}^p 3\lambda[j] \matkappa[j] \log \frac{3 md\matkappa[j]}{ \delta}\right),\\
			&\quad\le  \frac{12 mp \matkappa_1 }{\lambda_1}  \log \frac{3 md \matkappa_1}{ \delta} + \left(\frac{\nu}{\lambda_1}\right)^2 \cdot \frac{48m(p-d)\matkappa_2 }{\lambda_2}\log \frac{3 md\matkappa_2}{ \delta}. 
			\end{align*}
		\end{proof}
\end{comment}
